Training Aware Sigmoidal Optimizer

Proper optimization of deep neural networks is an open research question since an optimal procedure to change the learning rate throughout training is still unknown. Manually defining a learning rate schedule involves troublesome time-consuming try and error procedures to determine hyperparameters such as learning rate decay epochs and learning rate decay rates. Although adaptive learning rate optimizers automatize this process, recent studies suggest they may produce overffiting and reduce performance when compared to fine-tuned learning rate schedules. Considering that deep neural networks loss functions present landscapes with much more saddle points than local minima, we proposed the Training Aware Sigmoidal Optimizer (TASO), which consists of a two-phases automated learning rate schedule. The first phase uses a high learning rate to fast traverse the numerous saddle point, while the second phase uses low learning rate to slowly approach the center of the local minimum previously found. We compared the proposed approach with commonly used adaptive learning rate schedules such as Adam, RMSProp, and Adagrad. Our experiments showed that TASO outperformed all competing methods in both optimal (i.e., performing hyperparameter validation) and suboptimal (i.e., using default hyperparameters) scenarios.

==> algorithms/algorithm.tex <==
\begin{algorithm}%[!ht]
Initialize parameters;

\For{epoch $\gets$ 0 \textit{\textbf{to}} $epoch_{max}$}
{
	Choose a random input pattern $\boldsymbol{x}$;

	\eIf{\text{condition}}
    {
    	Run X;

    } {
    	Run Y.;
    }
}

\caption{Algorithm}
\label{alg:algorithm}
\end{algorithm}


==> algorithms/momentum.tex <==
\begin{algorithm}[!t]

\textbf{Require:} Learning rate $\epsilon$, momentum parameter $\alpha$

\textbf{Require:} Initial parameters $\theta$, initial velocity $v$

\While{stopping criterion not met}
{
	Sample a minibatch of $n$ examples from the training set $\{x^{(1)},\dots,x^{(n)}\}$ with corresponding targets $y^{(i)}$.
	
	Compute gradient estimate: $g \leftarrow + \nabla_\theta \sum_i L(f(x^{(i)}; \theta), y^{(i)})$ 
	
	Compute velocity update: $v \leftarrow \alpha v - \epsilon g$
	
	Apply update: $\theta \leftarrow \theta + v$

}

\caption{SGD with Momentum}
\label{alg:momentum}
\end{algorithm}


==> algorithms/nesterov.tex <==
\begin{algorithm}[!t]

\textbf{Require:} Learning rate $\epsilon$, momentum parameter $\alpha$

\textbf{Require:} Initial parameters $\theta$, initial velocity $v$

\While{stopping criterion not met}
{
	Sample a minibatch of $n$ examples from the training set $\{x^{(1)},\dots,x^{(n)}\}$ with corresponding targets $y^{(i)}$.
	
	Apply interim update: $\Tilde{\theta} \leftarrow \theta + \alpha v$
	
	Compute gradient (at interim point): $g \leftarrow + \nabla_\theta \sum_i L(f(x^{(i)}; \theta), y^{(i)})$ 
	
	Compute velocity update: $v \leftarrow \alpha v - \epsilon g$
	
	Apply update: $\theta \leftarrow \theta + v$

}

\caption{SGD with Nesterov Momentum}
\label{alg:nesterov}
\end{algorithm}


==> algorithms/sgd.tex <==
\begin{algorithm}[!t]

\textbf{Require:} Learning rate $\epsilon$

\textbf{Require:} Initial parameters $\theta$

\While{stopping criterion not met}
{
	Sample a minibatch of $n$ examples from the training set $\{x^{(1)},\dots,x^{(n)}\}$ with corresponding targets $y^{(i)}$.
	
	Compute gradient estimate: $g \leftarrow +\frac{1}{n} \nabla_\theta \sum_i L(f(x^{(i)}; \theta), y^{(i)})$ 
	
	Apply update: $\theta \leftarrow \theta -\epsilon g$

}

\caption{SGD}
\label{alg:sgd}
\end{algorithm}


==> figures/results/cifar100vggbestmanyruns.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=.98\linewidth]{figures/results/cifar100vggbestmanyruns.png}
	\caption{\textmd{Overall results for VGG19 on CIFAR100 using hyperparameters validated for VGG19 on CIFAR10. Shadow areas represent the variation of the many runs of the same experiment.}}
	\label{fig:cifar100_vgg_best_many_runs}
\end{figure}
